One-stage Video Instance Segmentation: From Frame-in Frame-out to Clip-in Clip-out

Many video instance segmentation (VIS) methods partition a video sequence into individual frames to detect and segment objects frame by frame. However, such a frame-in frame-out (FiFo) pipeline is ineffective to exploit the temporal information. Based on the fact that adjacent frames in a short clip are highly coherent in content, we propose to extend the one-stage FiFo framework to a clip-in clip-out (CiCo) one, which performs VIS clip by clip. Specifically, we stack FPN features of all frames in a short video clip to build a spatio-temporal feature cube, and replace the 2D conv layers in the prediction heads and the mask branch with 3D conv layers, forming clip-level prediction heads (CPH) and clip-level mask heads (CMH). Then the clip-level masks of an instance can be generated by feeding its box-level predictions from CPH and clip-level features from CMH into a small fully convolutional network. A clip-level segmentation loss is proposed to ensure that the generated instance masks are temporally coherent in the clip. The proposed CiCo strategy is free of inter-frame alignment, and can be easily embedded into existing FiFo based VIS approaches. To validate the generality and effectiveness of our CiCo strategy, we apply it to two representative FiFo methods, Yolact \cite{bolya2019yolact} and CondInst \cite{tian2020conditional}, resulting in two new one-stage VIS models, namely CiCo-Yolact and CiCo-CondInst, which achieve 37.1/37.3\%, 35.2/35.4\% and 17.2/18.0\% mask AP using the ResNet50 backbone, and 41.8/41.4\%, 38.0/38.9\% and 18.0/18.2\% mask AP using the Swin Transformer tiny backbone on YouTube-VIS 2019, 2021 and OVIS valid sets, respectively, recording new state-of-the-arts. Code and video demos of CiCo can be found at \url{https://github.com/MinghanLi/CiCo}.

==> fig/cis_sm.tex <==
\begin{figure*}[!t]
\begin{center}
    \includegraphics[width=0.95\linewidth]{fig/figs/clipvis_loss.jpg}
\end{center}
\vspace{-9mm}
\caption{Illustration of the clip-level instance masks generation process of CiCo-Yolact by a video in YouTube-VIS 2019. (a) A 4-frame input clip; (b) a subset of clip-level prototypes (only the six prototypes whose corresponding coefficients are greater than 0.75 are shown here); (c) clip-level instance masks of an object; and (d) the shared 32-dim mask parameters of the object ($k\!=\!32$).  }\label{fig:cis_sm}
\vspace{-2mm}
\end{figure*}

==> fig/length_of_clip.tex <==
\begin{figure*}[b]
\vspace{-3mm}
\begin{center}
\includegraphics[width=0.45\linewidth]{fig/figs/YT19.png}
\includegraphics[width=0.45\linewidth]{fig/figs/YT21_OVIS.png}
\end{center}
\vspace{-7mm}
\caption{
Ablation study of clip lengths for based-Yolact CiCo with different times of clip-level matcher $\psi=1$ and $\psi=3$.}\label{fig:length}
\vspace{-4mm}
\end{figure*}
